Focal Visual-Text Attention for Visual Question Answering

Recent insights on language and vision with neural networks have been successfully applied to simple single-image visual question answering. However, to tackle real-life question answering problems on multimedia collections such as personal photos, we have to look at whole collections with sequences of photos or videos. When answering questions from a large collection, a natural problem is to identify snippets to support the answer. In this paper, we describe a novel neural network called Focal Visual-Text Attention network (FVTA) for collective reasoning in visual question answering, where both visual and text sequence information such as images and text metadata are presented. FVTA introduces an end-to-end approach that makes use of a hierarchical process to dynamically determine what media and what time to focus on in the sequential data to answer the question. FVTA can not only answer the questions well but also provides the justifications which the system results are based upon to get the answers. FVTA achieves state-of-the-art performance on the MemexQA dataset and competitive results on the MovieQA dataset.

==> fvta_bak.tex <==
\section{Focal Visual-Text Attention}
%\subsection{Temporal Focal Pooling}
%In order to empower the network to learn to focus, the model should be able to capture the correlation between question and media documents at different timesteps.




\junwei{intuition of adding temporal pooling before attention}
The visual-text attention layer tries to let the model select related visual-text region or timestep based on each word of the question. We hypothesize that such fine-grained attention is difficult to learn. Meanwhile, most answers for personal collection questions are constrained and restricted in a short period of time, for example, "after dinner" or "what was the last time". Based on such observation, we introduce a \textbf{\textit{temporal focal pooling function}} to extract focal context representation before applying attention.

The focal context representation emphasizes relevant context hidden states based on the question. 
%To model the temporal dependency and cross-modal correlation in the visual-text sequence, 
First, we introduce a \textit{temporal correlation matrix}, $\mathbf{C} \in \mathbb{R}^{T \times T}$, a symmetric matrix where each entry $c_{ij}$ measures the correlation between context's the $i$-th step and the $j$-th step for a question. Let $\mathbf{h}_{i} = \mathbf{H}_{:i:} \in \mathbb{R}^{d \times 2}$ denote the visual/text representation for the $i$-th timestep in $\mathbf{H}$. For notation convince, $:$ is a slicing operator to extracts all elements from a dimension. 
%For example, $\mathbf{H}_{:i:}$ represents a new matrix. 
For example, $\mathbf{h}_{i1} = \mathbf{H}_{:i1}$ represents the vector representation of the $i$-th timestep of the visual sequence. 
Each entry $c_{ij}$ ($\forall i, j \in [1,T]$) in $\mathbf{C}$ is calculated by:

\begin{equation} \label{eq:time_w}
\begin{split}
c_{ij} &= \gamma(\mathbf{H}_{:i:},\mathbf{H}_{:j:},\mathbf{Q})  = \gamma(\mathbf{h}_{i},\mathbf{h}_{j},\mathbf{Q}) \\\
%&= \tanh\sum_{k=1}\mathbf{w}^\top_\mathbf{C}(\mathbf{h}^\top_{ik}\mathbf{h}_{jk}+\mathbf{w}^\top_{\mathbf{Q}}\mathbf{Q})
&= \tanh\sum_{k=1}^2 \mathbf{w}_c^\top(\mathbf{w}^\top_h[\mathbf{h}^\top_{ik}\odot\mathbf{h}_{jk} \| \\ &(\mathbf{h}_{ik}-\mathbf{h}_{jk})^\top\odot(\mathbf{h}_{ik}-\mathbf{h}_{jk})]+\mathbf{w}^\top_Q\mathbf{Q}), 
\end{split}
\end{equation}
where $\mathbf{w}_c$ , $\mathbf{w}_h$ and $ \mathbf{w}_{Q}$ are parameters to learn. $[\cdot \| \cdot ]$ represents a concatenation of two scalars\junwei{here should be vectors not scalars}vectors. The temporal correlation matrix captures the temporal dependency of question, image and text sequence. 
% explain why use the way of computation
In our work, we use the multiplication and subtraction of two vectors to represent the correlation since they are related to cosine similarity and Euclidean distance, respectively, and also preserve some information of the vectors by not summing up after the operation. It has been proven useful on text question-answering task~\cite{wang2016compare}.

To allow the model to capture connections between timesteps based on the question, we introduce temporal focal pooling to connect neighbouring time hidden states if they are related to the question, by utilizing the matrix $\mathbf{C}$.
For example, it can capture the relevance between the moment "dinner" and the moment later, "Went dancing", given the question "What did we do after the dinner on Ben's birthday?". 
%Now the matrix $\mathbf{C}$ obtains temporal context representation. We  
%$\mathbf{H}^{f}$ by a \textbf{\textit{temporal focal pooling function}} $g$:
Formally, given the time correlation matrix $\mathbf{C}$ and the context representation $\mathbf{H}$, we introduce a \textbf{\textit{temporal focal pooling function}} $g$ to obtain the focal representation $\mathbf{F} \in \mathbb{R}^{d \times T \times 2}$. Each vector entry $\mathbf{F}_{:tk}$ ($\forall t \in [1,T], \forall k \in [1,2]$) in $\mathbf{F}$ is calculated by:

%$\mathbf{h}_{ik},\mathbf{h}_{jk}$ are column vectors of $\mathbf{H}$ from $k$-th media document at timestep $i$ and $j$, respectively. 

\begin{equation} \label{eq:time_g}
\mathbf{F}_{:tk} = g(\mathbf{H};\mathbf{C},t,k) \in \mathbb{R}^{d}
\end{equation}

\begin{equation} \label{eq:time_g_h}
g(\mathbf{H};\mathbf{C},t,k) = \sum_{s}\mathbbm{1}[s \in [t-c,t+c]]\mathbf{C}_{st}\mathbf{h}_{tk}  
\end{equation}

\noindent where $\mathbf{F}_{:tk}$ is the focal context representation at $t$-th timesteps for $k$-th media. Since questions are usually about a specific short period of time, we constrain the model to only focus on a limited temporal window of contextual information with a trainable variable $c$.

\lu{lack insights why use the way to computet the C and F.}\junwei{explained in eq.4}
\begin{figure}[!t]
	\centering
		\includegraphics[width=0.47\textwidth]{tmm_comp_1dim_v2.png}
	\caption{\lu{redraw this graph. To illustrate our attention can capture the temporal dependency within a sequence and cross-modal interaction between texts and images.} 
	Comparison of the back-propagation of FVT attention and that of the classic soft attention mechanism. We argue that the traditional attention over this kind of visual-text, multi-level complex data collection is very hard to optimize.}
	\label{FVT_comp}
\end{figure}

%\subsection{Temporal Visual-Text Attention Tensor}


We apply attention over the focal context representation to summarize important information for answering the question.
We obtain the attention weights based on a correlation tensor $\mathbf{S}$ between each word of the question and each timestep of the visual-text sequences.
% Why introduce S, why attention is not a function of last attention
The attention at each timestep only considers the context and the question, and does not depend on the attention at previous timestep.
The intuition of using such a memory-less attention mechanism is that it simplifies the attention and let the model focus on learning the correlation between context and question. Such mechanism has been proven useful in text question answering~\cite{seo2016bidirectional}.
%Attention matrix $H$ allows for learning to focus on a few context regions. The regions vary for different  questions. To capture the correlation between question and visual-text sequences. 
We computes a \textit{kernel tensor}, $\mathbf{S} \in \mathbb{R}^{M \times T \times 2}$, between the input question and the focal context representation $\mathbf{F}$, where each entry in the kernel $s_{mtj}$ models the correlation between the $m$-th word in question and at $t$-th timestep over the modal $j$ (images or text words). Each entry $S_{mtj}$ in $\mathbf{S}$ is calculated by:

\begin{equation}    \label{eq:simi}
\begin{split}
s_{mtj} &= \kappa (\mathbf{F}_{:tj},\mathbf{Q}_{:m}) = \kappa(\mathbf{h},\mathbf{q}) \\
    &= \tanh(\mathbf{w^\top_s}[\mathbf{h} \odot \mathbf{q} \| (\mathbf{h}-\mathbf{q}) \odot (\mathbf{h}-\mathbf{q})] + \mathbf{b}_s)
\end{split}
\end{equation}
where $\kappa$ is a function to compute the correlation between question and context, $\mathbf{w}_s$ is the learned weights and $\mathbf{b}_s$ is the bias. $\odot$ is the element-wise multiplication and $[\cdot \| \cdot ]$ is vector concatenation across row. 
%The cosine function or a learned multi-layer perception can be used as kernel. In this paper, we find that a linear layer with concatenation of euclidean term and elem-wise multiplication on column vectors as shown in \cite{wang2016compare} works sufficiently well. 
As explained for Eq.~\ref{eq:time_w}, we use multiplication and subtraction to measure correlation between vectors since they capture both the cosine similarity and Euclidean distance information.
%\lu{I do not understand the notation. If it is matrix operation why there is subscripts?}
%\lu{Please revise the following formula. MAKE IT CLEARER. We will discuss them tomorrow.}
%\lu{No justification. Not clear why this operation will output attention tensor and why it help VQA over context sequences?}
%Focal Visual-Text Attention Tensor signifies the multi-dimensional relevancy between each timestep in context from different media documents and the question hidden representation. Given the question representation with time constraint (if any), temporal context attention tensor finds the importance of the representation at each timestep in each media. 
We obtain the visual-text sequence attention matrix $\mathbf{A} \in \mathbb{R}^{T \times 2}$ by: $\mathbf{A} = \max_{i=1}^M (\mathbf{S}_{i::})$ and the visual-text attention vector by $\mathbf{B}  \in \mathbb{R}^{2} = \max_{i=1}^T (\mathbf{A}_{i:})$. 
%using the temporal focal pooling operator $g$: % worse
%\begin{equation} \label{eq:time_att_full}
%a_{tj} = g(\max_{i=1}^M (\mathbf{S}_{i::});\mathbf{C},t,j)  \in \mathbb{R}
%\end{equation}
%\noindent where the maximum function $\max_{col}$ on $S$ is performed across the first column ($M$). Then the attended context vector is given by:
The maximum function $\max_{col}$ is performed across the first column. Then the attended context vector is given by:

%\lu{discuss how the implementation correspond to our motivation.}
\begin{equation} \label{eq:attend_h}
\mathbf{\tilde{h}} = \sum_{j=1}^2\mathbf{B}_{j} \sum_{t=1}^T \mathbf{A}_{tj}\mathbf{F}_{:tj} \in \mathbb{R}^{d}
\end{equation}
\junwei{intuition of using such attention}
The visual-text attention is computed based on the correlation between question and the focal context attention, which aligns with our observation that questions often provide constrains of a limited time window for the answers. 
To obtain the final context representation, we first summarize the focal context representation separately for visual sequence and text sequence, emphasizing the most important information using the intra-sequence attention.
Then, we obtain the final representation by summing the sequence vector representation based on the inter-sequence importance.


% move to related works
%\subsection{Comparison to other Attention Mechanism}
%Fig.~\ref{FVT_comp} illustrates the back-propagation flow difference between FVT attention tensor and one-dimensional question-to-context soft attention mechanism, along with the concatenate version of soft attention mechanism. Both mechanisms have the same amount of parameters but the attention weights are calculated differently. 
%We choose the MemexQA dataset to demonstrate the attention differences.
%In the soft attention, each word or photo in the visual-text sequences are used to compute the attention independently, hence the correlations of intra-sequence and inter-sequence are difficult to capture.
%One obvious modification would be to concatenate the corresponding sequences and apply attention on top, but it will lead to a hard constraint that the items in both sequences are either useful or not as shown in Fig. \ref{FVT_comp}.
%In FVTA, it first considers the inter-sequence relations with attention vector $\mathbf{B}$ and then the intra-sequence correlations with attention matrix $\mathbf{A}$. 
%With such mechanism of division of labor \junwei{divide and conquer?}, we argue that FVTA is able to capture the aforementioned correlations and is easier to optimize. 



\begin{comment}
\subsection{Context-aware Question vector}\lu{consider moving to supplementary materials}
We encode question representation $\mathbf{Q} \in \mathbb{R}^{d \times M}$ into a context-aware vector representation $\mathbf{\tilde{q}}$ with question-to-context attention $\mathbf{b} \in \mathbb{R}^{M}$, which is computed by:

\begin{equation} \label{eq:u_a}
\begin{split}
%\mathbf{b} = \max_{col^`}(\max_{col^`}(\mathbf{S})) \in \mathbb{R}^{M}
b_m &= \beta(\mathbf{\tilde{h}},\mathbf{Q}_{:m}) = \beta(\mathbf{\tilde{h}},\mathbf{q})\\
&=\tanh(\mathbf{w}^\top_b[\mathbf{\tilde{h}}\odot\mathbf{q}; (\mathbf{\tilde{h}} - \mathbf{q})\odot(\mathbf{\tilde{h}} - \mathbf{q})] + \mathbf{b}_b)
\end{split}
\end{equation}

\begin{equation} \label{eq:u_tilde}
\mathbf{\tilde{q}} = \sum_{m=1}^M b_m\mathbf{Q}_{:m} \in \mathbb{R}^{d}
\end{equation}

\noindent where $\mathbf{b}$ is the attention weights on the question words, and the maximum function $max_{col^`}$ operates across the last column.

\end{comment}
